Demystifying Compiler Unstable Feature Usage and Impacts in the Rust Ecosystem

Rust programming language is gaining popularity rapidly in building reliable and secure systems due to its security guarantees and outstanding performance. To provide extra functionalities, the Rust compiler introduces Rust unstable features (RUF) to extend compiler functionality, syntax, and standard library support. However, these features are unstable and may get removed, introducing compilation failures to dependent packages. Even worse, their impacts propagate through transitive dependencies, causing large-scale failures in the whole ecosystem. Although RUF is widely used in Rust, previous research has primarily concentrated on Rust code safety, with the usage and impacts of RUF from the Rust compiler remaining unexplored. Therefore, we aim to bridge this gap by systematically analyzing the RUF usage and impacts in the Rust ecosystem. We propose novel techniques for extracting RUF precisely, and to assess its impact on the entire ecosystem quantitatively, we accurately resolve package dependencies. We have analyzed the whole Rust ecosystem with 590K package versions and 140M transitive dependencies. Our study shows that the Rust ecosystem uses 1000 different RUF, and at most 44% of package versions are affected by RUF, causing compiling failures for at most 12%. To mitigate wide RUF impacts, we further design and implement a RUF-compilation-failure recovery tool that can recover up to 90% of the failure. We believe our techniques, findings, and tools can help to stabilize the Rust compiler, ultimately enhancing the security and reliability of the Rust ecosystem.

==> 8-discussion.tex <==
\section{Discussion}
\label{sec:discuss}

\noindent 
\textbf{Suggestions on Stabilizing RUF Implementation.}
For the Rust compiler, we suggest that the development process of the compiler should be systematically reconsidered.
The introduction of RUF can cause stability problems as it is now widely used and impacts the whole ecosystem, which makes the ecosystem less stable. What's worse, the RUF compatibility problems can make the whole package unusable for other developers, which is not friendly for maintainers and open source software community. 
First, we suggest that useless RUF should not be removed for compatibility concerns. If the RUF is not proven to be vulnerable or unstable, it can still work for developers, but with a warning instead.
Second, super-spreaders that a large number of packages depend on should avoid using RUF, especially when it is enabled by default. This can greatly eliminate RUF impacts in the Rust ecosystem.
Third, The Rust compiler should provide more information about RUF enabled to developers to build more reliable software.
% We recommend that the Rust team pay attention to compiler stability, especially the popular RUF, and try not to make new RUF public when it is still incomplete.

\noindent 
\textbf{Suggestions on Safely Using RUF.}
\loancold{Todo: Not complete}

Although the Rust ecosystem declares itself to be stable for developers, lots of packages will then face compilation failure caused by removed RUF.
To stabilize the Rust ecosystem, we recommend that developers (especially those who manage popular packages) backport their fixes to old versions. Following semantic versioning, dependent packages can automatically use fixed versions to avoid such failure. 
Moreover, to avoid RUF usage as much as possible, developers should use RUF only when it is inevitable. The RUF usage should be limited to a set of data structures and functions to be efficiently replaced in the future. 
What's more, developers should enable RUF only when it is needed. Developers can use RUF configuration predicates to declare environment and functionality requirements to enable RUF.
Last, we suggest that developers audit their dependencies to avoid using RUF as much as possible. They can select  

\noindent
\textbf{Extensibility of Our Technique.} \wenbo{open to public, seems too long}
\loancold{Only detailedly explain one extension, especially with contributions to the community.}
As shown in \cref{fig:impl_arch}, our proposed technique includes Rust compiler analysis, user program configuration extraction, and Ecosystem dependency graph resolution. Both the proposed technique and implementation are designed to be decoupled. This allows extended research work to be available in the future.

First, for packages outside the Rust ecosystem (data source extension), like personal projects and sub-projects, the dependency and program configuration analysis can lay the foundation for end-project analysis.
Second, for other ecosystem-level analysis via dependency (research area extension), based on our generated ecosystem dependency graph, vulnerability propagation, dependency conflict detection, ecosystem dependency graph evolution, and other ecosystem-level research can be easily and comprehensively conducted. We have successfully identified vulnerability impacts using our EDG by analyzing the whole ecosystem.
Third, for deeper investigation on compiler and ecosystem (technique extension), our technique is well documented with scripts and guidance and is open-source to the public. The unique technique proposed (each box in \cref{fig:impl_arch}) can be applied to other extensions. For example, our data-flow interception-based user configuration technique can be implemented to program configurations other than RUF, and the ecosystem dependency graph generator can be extended to analyze the dependency of compilation scripts with customized forms and types of dependencies considered.
In summary, we believe that the technique and tools in this paper can lay the foundation for further investigation on Rust.


% Although our dependency resolution process shows high accuracy, the dependencies of Rust projects outside the ecosystem and how developers use packages inside the ecosystem are still unknown in our analysis.
% We think there are three extra factors that need to be considered: Dependency lock, Different versions of toolchains, and Dependency entanglement.Moreover, we don't know which PF will be enabled and which platform users will run their programs on. As a result, we only give the range of RUF impacts rather than a precise one. 
% Aside from the ecosystem, we don't know how Rust applications use packages in the ecosystem, and how end users use Rust applications. 
% Our study only focuses on dependency resolution at the ecosystem level. As a result, to study the dependency network of all Rust projects and RUF impacts to end projects, we may need further investigation.

% Although Rust ecosystem declares itself to be stable and secure for developers, the dependency resolution process causes lots of packages to fail, because of yanked versions, dependency conflicts, etc. Moreover, lots of packages will then face failure caused by removed RUF.
% Stabilize the ecosystem.
% While previous work focus on threats in code-level threats, we point out that threats to Rust ecosystem should be taken seriously too.

% \begin{flushleft}
% \textbf{Further investigation using our tool.}
% As our tools are designed to be flexible, the dependency resolution in our tool can be easily adjusted to select different types of dependency information to support different impacts that can be introduced through dependency trees. Analysis of ecosystem can also depend on data given by our resolution. Other than Rust unstable features, impacts of vulnerabilities and other attributes inside a package can also be know using our generated ecosystem dependency graph.

% Although we systematically analyze the RUF usage and its impacts in Rust ecosystem, we don't know how to avoid its affection. To eliminate the impact RUF has caused to the ecosystem, we need to change the environment to avoid this. We can simply choose proper compiler version to make sure all RUF works, or choose package versions that works. There is still a lot of factors to be considered.
% \end{flushleft}

% \begin{flushleft}
% \textbf{Mitigating RUF impact through backporting.} 
% \end{flushleft}

% The technique proposed in this paper can also be further extended to other ecosystem-level analysis.

%In this paper, we analyze compiler unstable feature usage and impacts through dependency trees in the Rust ecosystem, achieved by an accurate and efficient dependency resolver and compiler static analyzer for unstable feature extraction. Our study constructs the dependency graph of Rust ecosystem and unstable feature usage information of all packages. Based on it, we have unveiled lots of useful findings and discussed the threats unstable feature causes to the entire ecosystem.

%\begin{acks}
%The authors would like to thank the associate editor and all reviewers sincerely for their valuable comments. This work is partially supported by the National Key R\&D Program of China (2022YFB3103900).
%\end{acks}


\subsection{Extensibility}


\subsection{Threat to Validity}


\subsection{Limitation}

% Resolution: Update Complexity + Accuracy outside the ecosystem

==> backup/3-impl.tex <==
\section{Implementation}
\loancold{Reshape the whole section.}

Now the implementation structure is still under consideration and will be modified later. However, we should write impl details in this section now.

\begin{figure*}[!t]
	\centering
	\includegraphics[width=0.80\textwidth]{pic/impl_arch.pdf}
	%\vspace{-5pt}
	\caption{The architecture of the analysis tool.}
	\label{fig:impl_arch}
\end{figure*}

\subsection{Dependency Resolution}
% Description in this subsection is poor. It doesn't clearly explain the implementation, making everything look mess.
% Second, consider other description format like Algorithm, data flow rather than simple architecture figure.

Official dependency resolution tool runs in single thread and needs Internet communication. The resolution results are not organized for large data operation. To perform large-scale ecosystem analysis, we have to design light-weight dependency resolution tool that is both efficient and accurate.

% However, achieving both efficiency and accuracy is challenging. Package managers including NPM, Maven and Cargo provide accurate resolution, but take seconds or minutes to complete. As a result, they can't be used to analyze the whole ecosystem in acceptable time. In previous work, they implement their own resolver to achieve efficiency (\loancold{need reference}), but they fail to cover all types of dependency making themselves less accuracy. To successful analyze the impact of RUF, we need to accurately resolve optional dependency and PF to find out how conditional RUF propagates in Rust ecosystem. This is harder as Cargo uses dependency cache mechanism and has dependency entanglement talked in ~\cref{dep_res}.

To achieve both efficiency and accuracy, we design our own resolver that reuses Cargo components shown in figure x. First, to achieve accuracy, we use the Cargo core resolver to resolve dependencies. However, the core resolver needs Cargo and package environment so that it can successfully recognize the dependency requirements. To conquer this problem, we build virtual environment for core resolver. The virtual package environment creates virtual dependency configuration that only contains target package to be resolved. The constructed Cargo environment virtualises its own Cargo environment rather than using the one in the host machine.

Second, to achieve efficiency at the same time, we change the interfaces where the core resolver gets data. Instead of fetching package metadata online from official database, we build a local copy and redirects online fetching into local. Also, to reduce I/O operations, we only store identifier of each package and necessary information rather than full output. At last, the resolution results are deduplicated into format of \textit{<VersionFrom, VersionTo, DepLevel, Addition>}. During resolution process, as we already provide independent virtual environment for each core resolver, resolvers won't lock each other as they update their own state rather than sharing one.

% Reserved: May be deleted or shortened.
Third, for flexibility of our resolver, our design allows customized query such as RUF analysis. In this way, our resolver can analyze other impacts in Rust ecosystem like vulnerability propagation. To achieve this, we \textit{double resolve} the virtual package. The first resolution process is intended to produce complete information like PF. Then, we change our package environment to specify extra requirements including PF, platform, blocked dependencies, etc. Then, the second resolution will output final results. With the help of Cargo components, we are able to get full information of the resolver. In this way, we can filter information we need, and store into the DB. 

The ecosystem dependency resolution process takes only about 1 day and produces over 100M indirect dependencies in a AlderLake machine.

\begin{algorithm}
    \caption{Rust Ecosystem Dependency Graph Generation}
    \label{alg:cap}
    \begin{algorithmic}[1]
        \Require $Q$ - Unresolved Packages
        \Ensure $G$ is Dependency Graph
        \State $G \gets \emptyset$
        \State $core\_resolver \gets new \ VirtualCargoEnv()$
        \ForEach{$ pack \in Q$}
            \State $cfg \gets new \ VirtualPackConfig()$
            \State $pre\_res \gets  core\_resolver.resolve(cfg)$
            \State $pack\_pf \gets  pre\_res.pf(pack) $
            \State $cfg.addPF(pack\_pf) $
            \State $res \gets  core\_resolver.resolve(cfg) $
            \ForEach{$ (dep\_pack, target\_pf, ruf) \in pack.ruf\_item$}
                \State $pf\_list \gets res.pf(dep\_pack)$
                \If{$target\_pf \in pf\_list$}
                    \State $G.push((dep\_pack, target\_pf, ruf))$
                \EndIf
            \EndFor
        \EndFor
        \State
        \Return $G$
    \end{algorithmic}
\end{algorithm}

\subsection{Rust Unstable Feature Extraction}

As we talked in \cref{ruf_analysis_challenge}, currently there is no such tools that can give out what RUF a package uses and under what condition the RUF is enabled. In fact, we are the first paper that focus on RUF and try to determine its impact. And thus, we have to develop new tools, which should be fast, accurate and easy to use.

Developing our tools from scratch is very difficult, especially when we have to parse the source code. So we decide to reuse the front-end of \textit{rustc} \cite{rustc:compiler} for reasons:
1) Accuracy. Since rustc is the official compiler, its parse result should be reliable.
2) Fast. Rustc uses a query-system \cite{rustc:query} based design, which accelerates the parsing process.
3) Developer-friendly. The structure design of rustc is very concise and elegant, while with relatively complete documentation \cite{rustc:dev_guide}.

Figure x shows how we reuse rustc: once rustc finishes the lexing and parsing processes, we intercept the data flow and analyze the raw data.

==> backup/5-evaluation.tex <==
\section{Accuracy Evaluation}

This is evaluation.

\begin{figure*}[!t]
	\centering
	\includegraphics[width=0.85\textwidth]{pic/eval_arch.pdf}
	%\vspace{-5pt}
	\caption{Dependency Resolution Accuracy Evaluation}
	\label{fig:eval_arch}
\end{figure*}

Experiment settings: We used toolchains including Cargo v1.2.3, and rust compiler v1.2.3-nightly.

\subsection{Standard Dependency Benchmark}

As different package manager uses different dependency resolution strategy, there is no standard resolution accuracy benchmark. For evaluation, we select \textit{Cargo Tree} tool from official package manager \textit{Cargo} for comparison. We resolute four types of dependency: Build, common, optional, target. Only development dependencies are omitted as they will not affect runtime of programs. Build scripts will be executed by default to create environment for runtime, like code and data. Common dependency are used for runtime. Optional dependencies and target-related dependencies are all considered as they are possibly used in real world.

~\cref{fig:eval_arch} describes the architecture of dependency resolution accuracy evaluation. We first download source code from official database \textit{Crates.io}, and then use \textit{Cargo Tree} to resolve dependencies in real environment. After that, we will compare dependency items from \textit{Cargo Tree} and our ecosystem dependency graph. 
We select 2\% packages from whole ecosystem as our standard dependency benchmark data set. To evaluate accuracy in different data set, we choose three strategies to select these packages: 1) Hot: Latest version of packages that has most downloads. 2) Mostdir: Latest version of packages that has most direct dependencies, which is the most complex situation a resolver will meet. 3) Random: Randomly select versions. 



\subsection{Dependency Resolution Accuracy Evaluation}

% Potential battle exists: Evaluation uses flat comparison rather than tree.

There are four types of results in the accuracy evaluation: 
1) $Right$: Dependency occurs in both dependency data set, with same versions. 
2) $Wrong$: Dependency occurs in both dependency data set, with wrong versions. 
3) $Over$: Dependency occurs in our resolution data set only.
4) $Miss$: Dependency occurs in standard data set only.

\sloppy We use 6 indexes to represent accuracy shown in \Crefrange{equa:TreeAcc}{equa:F1score}.
 $Tree Accuracy$ stands for resolution accuracy of entire dependency tree.
 $Recall$ and $Precision$ represents $Right$ in resolved dependencies and standard dependeny data set respectively.
%  $Critical Success Index$ (CSI)~\cite{wiki:Jaccard_index} represents the similarity and diversity of standard and our resolution results.
%  $Fowlkes-Malow Index$~\cite{eval:FM} and $F_{1}-score$~\cite{wiki:F-score} are geometric and harmonic mean of recall and precision respectively, and both of them can represent the accuracy of resolution.
$F_{1}-score$~\cite{wiki:F-score} is harmonic mean of recall and precision, which can represent the accuracy of resolution.
\begin{equation}\label{equa:TreeAcc}
         Tree Accuracy = \frac{Right Resolved Dependency Trees}{Resolved Dependency Trees} 
\end{equation}
\begin{equation}
         Recall = \frac{Right}{Right+Miss} 
\end{equation}
\begin{equation}
         Precision = \frac{Right}{Right+Wrong+Over}
\end{equation}
% \begin{equation}
%         Critical Success Index = \frac{Right}{Right+Wrong+Miss+Over}
% \end{equation}
% \begin{equation}
%          Fowlkes - Mallows Index = \sqrt{Recall*Precision}
% \end{equation}
\begin{equation}\label{equa:F1score}
         F_{1} - Score = \frac{2*Recall*Precision}{Recall+Precision}
\end{equation}

However, not all source code can be correctly resolved by \textit{Cargo Tree}. Some dependencies behave different when they are dependent on rather than direct resolution. The configuration file in the source code will force developers to use certain version of package manager, resolver and compiler. And it will also probably use local packages instead of packages from official database \textit{Crates.io}. This configuration setting is mostly used for local environments, but not for other developers who want to use the functionalities of this package. Because common developers using packages like this will not be affected by its configuration, our evaluation won't include the influence of configuration similar to this.

\begin{table}[]
    \caption{Resolution Accuracy}
    \label{tab:accuracy}
    \begin{tabular}{ccccc}
    \hline
    Dataset Type & Tree Accuracy & Precision & Recall  & F1Score \\ \hline
    Hot          & 99.23\%       & 99.99\%   & 98.14\% & 99.06\% \\
    Random       & 99.60\%       & 99.94\%   & 99.03\% & 99.48\% \\
    Mostdir      & 96.86\%       & 99.96\%   & 97.72\% & 98.83\% \\ \hline
    \end{tabular}
\end{table}

\subsection{Unstable Feature Extraction}

\loancold{We have to prove that our print path covers all types of unstable feature control flow to ensure 100\% accuracy. We can't use data set to evaluate extraction accuracy.}

\yinwhe{Still thinking about how to prove it.}

Evaluate our RUF extraction tool is quite challenging:
1) No ground truth. RUF is unique in rust programming language and there is no official tool or standard that we can use to validate our extraction results.
2) Lots of data. We can not evaluate manually since the number of versions is too big.

What we can do is 

\subsection{Threats to Validity}

This subsection may be removed.
